Low-Rank Tucker Approximation of a Tensor From Streaming Data

This paper describes a new algorithm for computing a low-Tucker-rank approximation of a tensor. The method applies a randomized linear map to the tensor to obtain a sketch that captures the important directions within each mode, as well as the interactions among the modes. The sketch can be extracted from streaming or distributed data or with a single pass over the tensor, and it uses storage proportional to the degrees of freedom in the output Tucker approximation. The algorithm does not require a second pass over the tensor, although it can exploit another view to compute a superior approximation. The paper provides a rigorous theoretical guarantee on the approximation error. Extensive numerical experiments show that that the algorithm produces useful results that improve on the state of the art for streaming Tucker decomposition.

==> conclusion.tex <==
\section{Conclusion}
\mnote{rewrite me}
This paper proposes a practical one-pass algorithm to compute the
Tucker decomposition of a tensor with provable guarantees.
Our algorithm uses a dimension reduction map to summarize the data in a linear sketch.
This sketch can be efficiently stored or transmitted, which enables applications in modern large-scale setting, including streaming and distributed data storage, or computational environment with limited memory.
We give the first comprehensive error analysis for one-pass Tucker decomposition algorithm in \cref{thm:low_rank_err}
and \cref{thm:fix_rank_err} for the tensor
approximation with error growing only linearly with the order $N$ of the tensor. In practice, our algorithm significantly outperforms the current state-of-the-art one-pass Tucker decomposition algorithm \cite{malik2018low} in the limited memory setting and noisy setting with much greater stability. Also, our one-pass achieves the same performance in \cite{malik2018low}'s suggested setting when the memory requirement is much higher than our suggested setting.
Our algorithm is available as an open-source python package.
% no acknowledgements in anonymous submission
% \subsubsection*{Acknowledgements}
% The authors would like to thank Guillaume Blanquart for discussing the applications of our sketching algorithm in combustion simulation data. The research is sponsored by ...

%\clearpage


==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage[numbers]{natbib}

\usepackage{bm}
\usepackage{stmaryrd}

\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\usepackage{dblfloatfix}
\usepackage[T1]{fontenc}
\usepackage{hyperref}
\usepackage{url}
\usepackage{booktabs}
\usepackage{amsfonts}
\usepackage{nicefrac}
\usepackage{microtype}
\usepackage[mathscr]{euscript}
\let\algorithmic\relax
\let\theoremstyle\relax
\RequirePackage{amsmath}
\usepackage{algorithm,algpseudocode}
\usepackage{color}
\usepackage{stmaryrd}
\usepackage{multirow}
\usepackage[titletoc,title]{appendix}
\usepackage{graphicx}

\usepackage{enumitem}
\usepackage{subcaption}
\usepackage{mathabx}
\usepackage{bbm}
\usepackage{float}
%\pdfsuppresswarningpagegroup=1

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


% \newcommand{\mnote}[1]{\textbf{[MU: #1]}}
% \newcommand{\jatnote}[1]{\textbf{[JAT: #1]}}
\newcommand{\mnote}[1]{}
\newcommand{\jatnote}[1]{}
\usepackage{tikz}
\usetikzlibrary{shapes.geometric}


\newcommand{\vc}{\mathop{\mathbf{vec}}}
\newcommand{\cov}{\mbox{Cov}}
\capstartfalse

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

\numberwithin{equation}{section}
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{assumption}{Assumption}
\newtheorem{prop}{Proposition}

%%% Madeleine's favorite shortcuts
% tensors
\newcommand{\T}[2][]{\boldsymbol{#1\mathscr{\MakeUppercase{#2}}}}
% matrices
\newcommand{\M}[1]{\mathbf{#1}}
% vectors
\newcommand{\V}[1]{\mathbf{#1}}
\newcommand{\E}{\mathbb{E}}

% linear algebra
\newcommand{\range}{\mathop{\textup{\bf{range}}}}

\newcommand{\cf}{cf.}
\newcommand{\eg}{e.g.}
\newcommand{\ie}{i.e.}
\newcommand{\etc}{etc.}

\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}


% Sets running headers as well as PDF title and authors
\headers{Low-Rank Tucker Approximation of a Tensor from Streaming Data}{Y. Sun, Y. Guo, C. Luo, J. Tropp, M. Udell}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Low-Rank Tucker Approximation of a Tensor from Streaming Data
\thanks{Submitted to the editors DATE.
%\funding{This work was funded by xxxx}
}}

% Authors: full names plus addresses.
\author{Yiming Sun\thanks{Cornell University, Ithaca
		(\email{ys784@cornell.edu}, \email{udell@cornell.edu}).}
	\and Yang Guo\thanks{University of Wisconsin-Madison, Madison, WI
		(\email{yguo@cs.wisc.edu}).}
	\and Charlene Luo\thanks{Columbia University, New York, NY (\email{cl3788@columbia.edu}).}
	\and
	Joel Tropp\thanks{California Institute of Technology, Pasadena, CA (\email{jtropp@cms.caltech.edu})}
	\and \mbox{Madeleine Udell}\footnotemark[2]
}



\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

\newcommand{\reals}{\mathbb{R}}



%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

